A Step Toward Deep Online Aggregation (Extended Version)

For exploratory data analysis, it is often desirable to know what answers you are likely to get before actually obtaining those answers. This can potentially be achieved by designing systems to offer the estimates of a data operation result -- say op(data) -- earlier in the process based on partial data processing. Those estimates continuously refine as more data is processed and finally converge to the exact answer. Unfortunately, the existing techniques -- called Online Aggregation (OLA) -- are limited to a single operation; that is, we cannot obtain the estimates for op(op(data)) or op(...(op(data))). If this Deep OLA becomes possible, data analysts will be able to explore data more interactively using complex cascade operations. In this work, we take a step toward Deep OLA with evolving data frames (edf), a novel data model to offer OLA for nested ops -- op(...(op(data))) -- by representing an evolving structured data (with converging estimates) that is closed under set operations. That is, op(edf) produces yet another edf; thus, we can freely apply successive operations to edf and obtain an OLA output for each op. We evaluate its viability with Wake, an edf-based OLA system, by examining against state-of-the-art OLA and non-OLA systems. In our experiments on TPC-H dataset, Wake produces its first estimates 4.93x faster (median) -- with 1.3x median slowdown for exact answers -- compared to conventional systems. Besides its generality, Wake is also 1.92x faster (median) than existing OLA systems in producing estimates of under 1% relative errors.

==> figures/data/II_approx_error_trend_WanderJoin.tex <==
%% WANDERJOIN RESULTS

% \pgfplotstableread{
% }\ScaleFiftyWanderJoinQueryThree

% \pgfplotstableread{
% }\ScaleFiftyWanderJoinQuerySeven

% \pgfplotstableread{
% }\ScaleFiftyWanderJoinQueryTen

==> figures/examples/double_axis.tex <==
\begin{figure*}[t]
    \centering
    \input{figures/data/II_approx_error_trend_data}

    \def\subplotwidthTwo{0.45\linewidth}
    \def\subplotwidthThree{0.30\linewidth}
    \pgfplotsset{
        accfig/.style={
            height=30mm,
            width=\linewidth,
            % xmode=log,
            % ymode=log,
            axis lines=left,
            enlarge x limits=0.1,
            enlarge y limits=0.1,
            xlabel=Elapsed Time (s),
            xlabel near ticks,
            ylabel=MAPE (\%),
            ylabel near ticks,
            ylabel style={align=center},
            legend style={
                at={(0.5,1.05)},anchor=south,column sep=2pt,
                draw=black,fill=white,line width=.5pt,
                font=\scriptsize,
                /tikz/every even column/.append style={column sep=5pt}
            },
            legend columns=2,
            colormap name=bright,
            every axis/.append style={font=\footnotesize},
            every non boxed x axis/.append style={x axis line style=-},
            xmajorgrids,
            ymajorgrids,
            ylabel near ticks,
        },
        accfig/.belongs to family=/pgfplots/scale,
    }
    \begin{subfigure}[b]{\subplotwidthThree}
        \centering
        \begin{tikzpicture}
            \begin{axis}[
                accfig,
                axis y line*=left,
                ylabel=MAPE (\%),
            ]
            
                \addplot[mark=diamond, color={wakecolor}, mark repeat=20]
                table[x=time_avg_s,y=mape_p] {\powerHundredqXXIII}; \label{fig:II_accuracy_rp_curve_A_mape}

            \end{axis}
            
            \begin{axis}[
                accfig,
                axis y line*=right,
                axis x line=none,
                ylabel=Recall or Precision (\%),
            ]
                \addlegendimage{/pgfplots/refstyle=fig:II_accuracy_rp_curve_A_mape}\addlegendentry{MAPE}
            
                \addplot[mark=x, color={wakerecallcolor}, mark repeat=20]
                table[x=time_avg_s,y=recall_p] {\powerHundredqXXIII}; \addlegendentry{Recall}
            
                \addplot[mark=o, color={wakeprecisioncolor}, mark repeat=20]
                table[x=time_avg_s,y=precision_p] {\powerHundredqXXIII}; \addlegendentry{Precision}
            
            \end{axis}
        \end{tikzpicture}
        % \vspace{-2mm}
        \caption{Modified Q3}  % q23
        \label{fig:II_accuracy_curve_3_q3}
    \end{subfigure}
    \vspace{-2mm}
    \caption{Approximation error, recall, and precision over time compared. Vertical lines represent completion time of exact methods.}
    \label{fig:II_accuracy_rp_curve}
\end{figure*}


==> figures/examples/errorbar_subplots.tex <==
% This generates many subplots of bar plots with errors. Subplots have different widths. Each subplot also has an arrow pointing to highlight a "solution".

\begin{figure*}[t]

\pgfplotsset{
    accfig/.style={
        width=\linewidth,
        height=35mm,
        ybar,
        axis lines=left,
        bar width=1.6mm,
        bar shift=0pt,
        enlarge x limits=0.1,
        xlabel=Number of Layers $L$, 
        ylabel near ticks,
        ylabel style={align=center},
        xlabel style={yshift=0mm},
        xticklabel style={font=\scriptsize, text width=5mm, align=center},
        legend style={
            at={(1.02,1.00)},anchor=north west,column sep=2pt,
            draw=black,fill=white,line width=.5pt,
            /tikz/every even column/.append style={column sep=5pt}
        },
        legend cell align={left},
        legend columns=1,
        area legend,
        clip=false,
        every axis/.append style={
            font=\footnotesize
        },
        /pgfplots/log origin=infty,
        xtick style={draw=none},
        xtick pos=bottom,
        minor tick num=1,
        minor grid style=lightgray,
        ymajorgrids,
        yminorgrids,
        },
    accfig/.belongs to family=/pgfplots/scale,
}

\begin{subfigure}[t]{0.2\linewidth} \centering
    \begin{tikzpicture}
    
    \begin{axis}[accfig,
        ymin=0,
        ymax=290,
        xtick={1, ..., 5},
        xticklabels={
            1,
            2,
            3, 
            4, 
            5, 
        },
        ylabel=Search Latency (ms)]
    
    \addplot[fill={airindexcolor}]
    plot [error bars/.cd, y dir=both,y explicit,error bar style={color=black}]
    table[x=x,y=y, y error=std] { 
    x y std
    1 69.64 20.39
    };
    
    \addplot[fill={btreecolor}]
    plot [error bars/.cd, y dir=both,y explicit,error bar style={color=black}]
    table[x=x,y=y, y error=std] { 
    x y std
    2 94.62 21.22
    3 120.78 34.81
    4 155.78 62.75
    5 190.77 65.34
    };
    
    \node[font=\scriptsize,anchor=south west,draw=airindexcolor,text=airindexcolor,
        thick,fill=white]  (O)
        at (axis cs: 0.8, 200) 
        {\textbf{\textsf{Tuned}}};
    \draw [to-,ultra thick,airindexcolor] (axis cs: 1,140) -- (1,200);
      
    \end{axis}
    
    \end{tikzpicture}
    \vspace{-2mm}
    \caption{Varying $L$ on NFS}
\end{subfigure}
~
\begin{subfigure}[t]{0.3\linewidth} \centering
    \begin{tikzpicture}
    
    \begin{axis}[accfig,
        ymin=0,
        ymax=290,
        ylabel=Search Latency (ms),
        xtick={1, 2, ..., 8},
        xticklabels={
            $2^{8}$, 
            $2^{10}$,
            $2^{12}$, 
            $2^{14}$, 
            $2^{16}$, 
            $\mathbf{2^{16.3}}$,
            $2^{18}$, 
            $2^{20}$, 
        },
        xlabel=Granularity $\lambda$]
    
    \addplot[fill={airindexcolor}]
    plot [error bars/.cd, y dir=both,y explicit,error bar style={color=black}]
    table[x=x,y=y, y error=std] { 
    x y std
    6 69.64 20.39
    };
    
    \addplot[fill={btreecolor}]
    plot [error bars/.cd, y dir=both,y explicit,error bar style={color=black}]
    table[x=x,y=y, y error=std] { 
    x y std
    1 149.92 40.92
    2 112.46 35.64
    3 107.57 25.33
    4 89.64 25.90
    5 76.37 19.62
    7 76.50 26.46
    8 73.69 17.28
    };
    
    \node[font=\scriptsize,anchor=south west,draw=airindexcolor,text=airindexcolor,
        thick,fill=white]  (O)
        at (axis cs: 4.8, 200) 
        {\textbf{\textsf{Tuned}}};
    \draw [to-,ultra thick,airindexcolor] (axis cs: 6,140) -- (6,200);
    
    \end{axis}
    \end{tikzpicture}
    \vspace{-2mm}
    \caption{Varying $\lambda$ on NFS}
\end{subfigure}
~
\begin{subfigure}[t]{0.2\linewidth} \centering
    \begin{tikzpicture}
    
    \begin{axis}[accfig,
        xtick={1, ..., 5},
        xticklabels={
            1, 
            2,
            3, 
            4, 
            5, 
        },
        ymin=0,
        ymax=7.9,
        ylabel=Search Latency (ms)]
    
    \addplot[fill={airindexcolor}]
    plot [error bars/.cd, y dir=both,y explicit,error bar style={color=black}]
    table[x=x,y=y, y error=std] { 
    x y std
    2 2.90 0.52
    };
    
    \addplot[fill={btreecolor}]
    plot [error bars/.cd, y dir=both,y explicit,error bar style={color=black}]
    table[x=x,y=y, y error=std] { 
    x y std
    1 3.02 0.43
    3 3.83 0.87
    4 4.83 0.99
    5 5.49 1.92
    };
    
    \node[font=\scriptsize,anchor=south west,draw=airindexcolor,text=airindexcolor,
        thick,fill=white]  (O)
        at (axis cs: 1.3, 6) 
        {\textbf{\textsf{Tuned}}};
    \draw [to-,ultra thick,airindexcolor] (axis cs: 2,4) -- (2,6);
    
    \end{axis}
    \end{tikzpicture}
    \vspace{-2mm}
    \caption{Varying $L$ on SSD}
\end{subfigure}
~
\begin{subfigure}[t]{0.3\linewidth} \centering
    \begin{tikzpicture}
    
    \begin{axis}[accfig,   
        ymin=0,
        ymax=7.9,
        xtick={1, 2, ..., 8},               
        xticklabels={
            $2^{8}$, 
            $2^{10}$,
            $\mathbf{2^{11.6}}$,
            $2^{12}$, 
            $2^{14}$, 
            $2^{16}$, 
            $2^{18}$, 
            $2^{20}$, 
        },
        xlabel=Granularity $\lambda$,
        ylabel=Search Latency (ms)]
    
    \addplot[fill={airindexcolor}]
    plot [error bars/.cd, y dir=both,y explicit,error bar style={color=black}]
    table[x=x,y=y, y error=std] { 
    x y std
    3 2.90 0.52
    };
    
    \addplot[fill={btreecolor}]
    plot [error bars/.cd, y dir=both,y explicit,error bar style={color=black}]
    table[x=x,y=y, y error=std] { 
    x y std
    1 4.18 0.48
    2 3.85 1.59
    4 3.10 1.30
    5 2.67 0.85
    6 3.00 0.91
    7 2.68 0.82
    8 3.19 0.89
    };
    
    \node[font=\scriptsize,anchor=south west,draw=airindexcolor,text=airindexcolor,
        thick,fill=white]  (O)
        at (axis cs: 2.3, 6) 
        {\textbf{\textsf{Tuned}}};
    \draw [to-,ultra thick,airindexcolor] (axis cs: 3,4) -- (3,6);
      
    \end{axis}
    \end{tikzpicture}
    \vspace{-2mm}
    \caption{Varying $\lambda$ on SSD}
\end{subfigure}
    
    \vspace{-3mm}
    \caption{Comparison between \system-tuned designs (in red) and manual alternatives across NFS and SSD (\texttt{fb} dataset) varying the number of layers $L$ and the granularity hyperparameter $\lambda$. The error bars display standard deviations of the latency.}
    \vspace{-3mm}
    \label{fig:III_variants}
\end{figure*}


==> figures/examples/stackedbarplot.tex <==
% Horizontally stacked bar plot. Add more "breakdowns" by adding more columns to the table + add more \addplot + add legend label

\begin{figure}[t]

\pgfplotstableread{
method wait download
lucene 859.6774193548387 211.93548387096777
elasticsearch 909.0 572.5
sqlite 629.032258064516 165.1612903225806
hashtable 370.0 817.0967741935484
iou0 220.33333333333331 116.66666666666666
}\dataTransferTable

\centering
\begin{tikzpicture}
    \begin{axis}[
        xbar stacked,
        scale only axis,
        bar width=1.8mm,
        width=0.75\linewidth,
        height=0.25\linewidth,
        xmin=0,
        xmax=2000,
        xtick={0, 500, ..., 2000},
        minor tick num=1,
        xmajorgrids,
        xminorgrids,
        y dir=reverse,
        ytick=data,
        xlabel near ticks,
        ylabel near ticks,
        xlabel=Latency (ms),
        xlabel shift=-1mm,
        yticklabels={Lucene,Elasticsearch,SQLite,HashTable,\system},
        every axis/.append style={font=\scriptsize},
        legend style={
            font=\scriptsize,
            at={(0.98,0.05)}, anchor=south east,
            draw=black,
            fill=white
        },
        legend cell align={left},
    ]
        \addplot [
            fill=vintageblack!70
        ] table [x=wait, meta=method,y expr=\coordindex] {\dataTransferTable};
        
        \addplot [
            fill=vintageblack!10,
        ] table [x=download, meta=method,y expr=\coordindex] {\dataTransferTable};
        
        \legend{Wait Time,Download Time}
    \end{axis}
\end{tikzpicture}
\vspace{-2mm}

\caption{Search latency breakdown in terms of network communication on the \texttt{Spark} dataset. The total search latency is equal to the summation of wait time and download time.}
\vspace{-2mm}

\label{fig:data_transfer}
\end{figure}


==> figures/experiments/II-1_wake_approx_error_trend.tex <==
\begin{figure*}[ht]
    \centering
    \input{figures/data/II_approx_error_trend_data}

    \def\subplotwidthTwo{0.45\linewidth}
    \def\subplotwidthThree{0.25\linewidth}
    \def\height{32mm}
    \def\hspaceGap{5mm}
    \pgfplotsset{
        accfigLeft/.style={
            height=\height,
            width=\linewidth,
            % xmode=log,
            ymode=log,
            axis y line*=left,
            enlarge x limits=0.1,
            % enlarge y limits=0.1,
            xlabel=Elapsed Time (s),
            xlabel near ticks,
            ylabel=MAPE (\%),
            ylabel near ticks,
            ylabel style={align=center},
            legend columns=2,
            colormap name=bright,
            every axis/.append style={font=\footnotesize},
            xmajorgrids,
            ymajorgrids,
            ylabel near ticks,
        },
        accfigLeft/.belongs to family=/pgfplots/scale,
    }
    \pgfplotsset{
        accfigRight/.style={
            height=\height,
            width=\linewidth,
            % xmode=log,
            % ymode=log,
            axis x line=none,
            axis y line*=right,
            enlarge x limits=0.1,
            % enlarge y limits=0.1,
            ymin=0.0,
            ymax=100.0,
            xlabel=Elapsed Time (s),
            xlabel near ticks,
            ylabel={Recall (\%)},
            ylabel near ticks,
            ylabel style={align=center},
            legend style={
                % at={(0.5,1.05)},anchor=south,column sep=2pt,
                at={(1.45,0.5)},anchor=west,column sep=2pt,
                draw=black,fill=white,line width=.5pt,
                font=\scriptsize,
                /tikz/every even column/.append style={column sep=5pt}
            },
            % legend columns=3,
            legend columns=1,
            colormap name=bright,
            every axis/.append style={font=\footnotesize},
            every non boxed x axis/.append style={x axis line style=-},
            xmajorgrids,
            ymajorgrids,
            ylabel near ticks,
        },
        accfigRight/.belongs to family=/pgfplots/scale,
    }
    \begin{subfigure}[b]{\subplotwidthThree}
        \centering
        \begin{tikzpicture}
            \begin{axis}[
                accfigLeft
            ]
                \addplot[mark=diamond, color={wakecolor}, thick, mark repeat=20]
                table[x=time_avg_s,y=mape_p] {\powerHundredqIX}; \label{fig:II_accuracy_rp_curve_A_mape}
            \end{axis}
            
            \begin{axis}[
                accfigRight
            ]
                % \addlegendimage{/pgfplots/refstyle=fig:II_accuracy_rp_curve_A_mape}\addlegendentry{MAPE}
            
                % \addplot[mark=o, color={wakeprecisioncolor}, mark repeat=20]
                % table[x=time_avg_s,y=precision_p] {\powerHundredqIX};
                % % \addlegendentry{Precision}
            
                \addplot[mark=x, color={wakerecallcolor}, thick,  mark repeat=20]
                table[x=time_avg_s,y=recall_p] {\powerHundredqIX};
                % \addlegendentry{Recall}
            \end{axis}
        \end{tikzpicture}
        \caption{Q9}
        \label{fig:II_accuracy_rp_curve_1_q9}
    \end{subfigure}
    \hspace{\hspaceGap}
    \begin{subfigure}[b]{\subplotwidthThree}
        \centering
        \begin{tikzpicture}
            \begin{axis}[
                accfigLeft,
                ymode=linear,
                ymin=0.0,
                ymax=100.0,
            ]
                \addplot[mark=diamond, color={wakecolor}, thick, mark repeat=20]
                table[x=time_avg_s,y=mape_p] {\powerHundredqXVIII}; \label{fig:II_accuracy_rp_curve_B_mape}
            \end{axis}
            
            \begin{axis}[
                accfigRight
            ]
                % \addlegendimage{/pgfplots/refstyle=fig:II_accuracy_rp_curve_B_mape}\addlegendentry{MAPE}
            
                % \addplot[mark=o, color={wakeprecisioncolor}, mark repeat=20]
                % table[x=time_avg_s,y=precision_p] {\powerHundredqXVIII};
                % % \addlegendentry{Precision}
            
                \addplot[mark=x, color={wakerecallcolor}, thick, mark repeat=20]
                table[x=time_avg_s,y=recall_p] {\powerHundredqXVIII};
                % \addlegendentry{Recall}
            \end{axis}
        \end{tikzpicture}
        \caption{Q18}
        \label{fig:II_accuracy_rp_curve_2_q18}
    \end{subfigure}
    \hspace{\hspaceGap}
    \begin{subfigure}[b]{\subplotwidthThree}
        \centering
        \begin{tikzpicture}
            \begin{axis}[
                accfigLeft
            ]
                \addplot[mark=diamond, color={wakecolor}, thick, mark repeat=5]
                table[x=time_avg_s,y=mape_p] {\powerHundredqXXI}; \label{fig:II_accuracy_rp_curve_C_mape}
            \end{axis}
            \begin{axis}[
                accfigRight
            ]
                \addlegendimage{/pgfplots/refstyle=fig:II_accuracy_rp_curve_C_mape}\addlegendentry{MAPE}
            
                % \addplot[mark=o, color={wakeprecisioncolor}, mark repeat=5]
                % table[x=time_avg_s,y=precision_p] {\powerHundredqXXI};
                % \addlegendentry{Precision}
            
                \addplot[mark=x, color={wakerecallcolor}, thick, mark repeat=5]
                table[x=time_avg_s,y=recall_p] {\powerHundredqXXI};
                \addlegendentry{Recall}
            \end{axis}
        \end{tikzpicture}
        \caption{Q21}
        \label{fig:II_accuracy_rp_curve_3_q13}
    \end{subfigure}
    \hfill
    \vspace{-2mm}
    \caption{Approximation Error and Recall compared over time. Vertical lines represent completion time of exact methods. \supawit{TODO: add vertical lines}}
    \label{fig:II_accuracy_rp_curve}
\end{figure*}


==> figures/experiments/II-2_pdb_approx_error_trend.tex <==
\begin{figure*}[ht]
    % \centering
    \input{figures/data/II_approx_error_trend_pdb}
    \input{figures/data/II_approx_error_trend_data}

    \def\subplotwidthTwo{0.30\linewidth}
    \def\subplotwidthThree{0.30\linewidth}
    \pgfplotsset{
        accfig/.style={
            height=32mm,
            width=52mm,
            xmode=log,
            ymode=log,
            axis lines=left,
            enlarge x limits=0.1,
            enlarge y limits=0.05,
            xlabel=Elapsed Time (s),
            xlabel near ticks,
            ylabel=MAPE (\%),
            ylabel near ticks,
            ylabel style={align=center},
            legend style={
                at={(1.2, 0.5)},anchor=west,column sep=2pt,
                draw=black,fill=white,line width=.5pt,
                font=\scriptsize,
                /tikz/every even column/.append style={column sep=5pt}
            },
            legend columns=1,
            colormap name=bright,
            every axis/.append style={font=\footnotesize},
            xmajorgrids,
            ymajorgrids,
            ylabel near ticks,
        },
        accfig/.belongs to family=/pgfplots/scale,
    }
    
    % \hspace{-64mm}
    \begin{subfigure}[b]{\subplotwidthTwo}
        % \centering
        \begin{tikzpicture}
            \begin{axis}[
                accfig,
                ymin=0.001
            ]
            
            % \addplot+[mark=x, color={prestocolor}, mark repeat=20]
            % table[x=time,y=acc] {\qaTable};
            % % \addlegendentry{\presto}
            
            % \addplot+[mark=o, color={polarcolor}, mark repeat=20]
            % table[x=time,y=acc] {\qaTable};
            % % \addlegendentry{\polar}
            
            \addplot+[mark=square, color={progressivedbcolor}, thick, mark repeat=20]
            table[x=time_avg_s,y=mape_p] {\pdbHundredqI};
            % \addlegendentry{\postgres}
            
            \addplot+[mark=diamond, color={wakecolor}, thick, mark repeat=20]
            table[x=time_avg_s,y=mape_p] {\powerHundredqXXVI};
            % \addlegendentry{\system}
            
            % \addplot+[mark=diamond, color={noscalecolor}, mark repeat=20]
            % table[x=time_avg_s,y=mape_p] {\vanillaHundredqI};
            % % \addlegendentry{\noscale}
            
            \node[draw=black, fill=white, anchor=north east, align=right, font=\scriptsize\sf] at (rel axis cs:1.00,1.00) {Modified Q1};
            
            \end{axis}
        \end{tikzpicture}
        % \label{fig:II_accuracy_curve_1_q1}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{\subplotwidthTwo}
        \begin{tikzpicture}
            \begin{axis}[
                accfig,
                ymin=0.0001,
                ytick={0.0001, 0.01, 1, 100},
            ]
            
            % \addplot+[mark=x, color={prestocolor}, mark repeat=20]
            % table[x=time,y=acc] {\qaTable};
            % % \addlegendentry{\presto}
            
            % \addplot+[mark=o, color={polarcolor}, mark repeat=20]
            % table[x=time,y=acc] {\qaTable};
            % % \addlegendentry{\polar}
            
            \addplot+[mark=square, color={progressivedbcolor}, thick, mark repeat=20]
            table[x=time_avg_s,y=mape_p] {\pdbHundredqVI};
            \addlegendentry{\progressivedb}
            
            \addplot+[mark=diamond, color={wakecolor}, thick, mark repeat=20]
            table[x=time_avg_s,y=mape_p] {\powerHundredqXXVII};
            \addlegendentry{\system}
            
            % \addplot+[mark=diamond, color={noscalecolor}, mark repeat=20]
            % table[x=time_avg_s,y=mape_p] {\vanillaHundredqVI};
            % \addlegendentry{\system Manual Power}
            
            \node[draw=black, fill=white, anchor=north east, align=right, font=\scriptsize\sf] at (rel axis cs:1.00,1.00) {Modified Q6};
            
            \end{axis}
        \end{tikzpicture}
        % \label{fig:II_accuracy_curve_2_q6}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.38\linewidth}
    \hphantom{hello}
    \end{subfigure}
    
    \vspace{-4mm}
    \caption{Approximation error over time on Q1 and Q6 
        modified to be compatible with \progressivedb.}
    \label{fig:II_accuracy_curve_progressivedb}
\end{figure*}


==> figures/experiments/III_breakdown.tex <==
% Breakdown by node and active execution interval

==> figures/experiments/V_discrete_accuracy.tex <==
% time to x% error across many queries

==> figures/fig_operations.tex <==
\begin{table*}[t]

\caption{Mutation type changes by operations.
The first column is pre-op type, the header (first row) is applied operations,
    and the other cells are post-op types. *ck stands for clustering key.}
\vspace{-2mm}

\centering
\small
\begin{tabular}{ c | c c c c c c }
\toprule
                & map & join on ck$^*$ & agg by ck$^*$ & agg by non-ck & filter on const\_attr & filter on mutable\_attr \\ \midrule 
\textbf{Type-A} & A   & A              & A             & M             & A               & n/a                   \\  
\textbf{Type-M} & M   & M              & M             & M             & M               & M                     \\ \bottomrule
\end{tabular}
\end{table*}


==> figures/tables/wake-nodes.tex <==
\begin{table}[t]
\begin{center}
\caption{Node types implemented in \system}
\label{tab:wake-node-operations}
\vspace{-2mm}
\small
\begin{tabular}{ l | l }
\toprule
\textbf{node type} & \textbf{description} \\ 
\midrule
reader & Read tables in different formats \\
appender & Single input channel map operations (and filter) \\
map-merger & Dual input channel map operations\\
hash-join & Performing hash-join with right channel in memory \\
sorted-join & Performing join on dataframes sorted on the join-key \\
aggregator & For performing group-by aggregation \\
accumulator & For blocking accumulating operations \\
\bottomrule
\end{tabular}
\end{center}
\end{table}


==> sections/2-2_background.tex <==
% This table is for the background section (Section 2)
\input{figures/table_previous_work}

\newpage

\section{Template-Based Online Aggregation}


\begin{enumerate}
\item hard to handle joins
\item hard to handle subqueries
\item unclear how to further process approximate result sets
\item Confusing notion: to process a table that continuously updates
\end{enumerate}



==> sections/5-2_draft.tex <==


\system models group cardinality as a multinomial distribution with time-dependent parameters:

\begin{equation}
\begin{split}
\bfX(t) \; | \; n(t), \bfp(t)
    & \sim \text{Multinomial}(n(t), \bfp(t)) \\
\bfp(t)
    & \sim \text{Dirichlet}(\bfq(t))
\end{split}
\end{equation}

where $\bfX(t) = [X_1(t), \dots, X_M(t)]$, $\bfp(t) = [p_1(t), \dots, p_M(t)]$, and $\bfq(t) = [q_1(t), \dots, q_M(t)]$ are vectorized group cardinalities, multinomial event probabilities, and Dirichlet concentration parameters. Because Dirichlet distribution is a conjugate prior to multinomial distribution, we have that $\bfp(t) | \bfX(t) \sim \text{Dirichlet}(\bfX(t))$~\cite{???}.

where $M = \max_t m(t)$ is the total number of groups, $n(t)$ is the number of samples up until progress $t$, and $(p_1(t), \dots, p_M(t))$ follows a Dirichlet prior with time-dependent parameters $(q_1(t), \dots, q_M(t))$.

$$q_i(t) = c_i t^{u - v}$$

$$c_i = \frac{x_{i, t}}{t^{u - v}}, N = \frac{n(t)}{t^{u}}, M = \frac{m(t)}{t^{v}}$$

consistency at $t$: $\sum_{i=1}^{m(t)} q_i(t) = \sum_{i=1}^{m(t)} x_{i, t} = n(t)$

consistency at $T$: $\sum_{i=1}^{m(t)} q_i(T) = \sum_{i=1}^{m(t)} \frac{x_{i, t}}{t^{u - v}} = \frac{n(t)}{t^{u - v}} < \frac{n(t)}{t^{u}} = N$. The other $\frac{n(t)}{t^{u}} - \frac{n(t)}{t^{u - v}} = \frac{n(t) (1 - t^{v})}{t^{u}}$ are unobserved.

%$p_i(t) = c_i \frac{n(t)}{m(t)} = \frac{c_i N}{M} t^{u - v}$.

% By multinomial constraint on $p_i(t)$, $z(t) = \sum_{i=1}^{m(t)} c_i$.



% Note that $N = n(T)$ is the final number of samples and so $\sum_{i=1}^{m(t)} x_{i, t} = n(t)$.


$\sum_{i=1}^{m(t)} c_i = a m(t)$

$m(t) = s_i t^{r_i}$

Problem: ordering in group?

$\frac{1}{m(t)} \sum_{i=1}^{m(t)} x_{i, t} = \frac{n(t)}{m(t)}$

Try 3:

% Assume stochastically categorical and multinomial distribution
% \begin{enumerate}
%     \item Draw $m(t)$ groups, unequal probability, $M(t)$
%     \item Draw multinomial distribution $X_t(t) \sim \text{Multi}(p_1(t), \dots, p_m(t))$
% \end{enumerate}

Assume stochastic multinomial distribution, s.t. $\sum_{i=1}^{m(t)} p_i(t) = 1, \forall t$

$$X(t) \sim \text{Multi}(p_1(t), \dots, p_m(t))$$

$$p_i(t) = a_i t^p + b_i$$

Guess: $p_i(t) = \frac{a_i t^p + b_i}{\sum_{i=1}^m a_i t^p + b_i}$

Maybe shared coefficient $a_i = a$?

\begin{align*}
    & \sum_{i=1}^{m} a_i t^p + b_i = 1 \\
\end{align*}

Try 2:

Assume stochastic multinomial distribution, s.t. $\sum_{i=1}^{m(t)} p_i(t) = 1, \forall t$

$$g(t) \sim \text{Multi}(p_1(t), \dots, p_m(t))$$

$$p_i(t) = c_i \frac{n(t)}{m(t)} = c_i \frac{N t}{N t^{1-p}} = \frac{c_i t^p}{\sum_{i=1}^{m(t)} c_i t^p}$$

\begin{align*}
    & \sum_{i=1}^{m(t)} c_i t^p = 1 \\
    & \sum_{i=1}^{m(t)} c_i = \frac{1}{t^p} \\
\end{align*}


MLE:

\begin{align*}
    \max_{c_1, \dots, c_m, p} \prod_{t} n(t)! \prod_{i=1}^m \frac{p_i(t)^{x_{i, t}}}{x_{i, t}!}
\end{align*}

MLLE $\theta = (c_1, \dots, c_m, p, \lambda_t), \forall t$

\begin{align*}
    & \max_{\theta} \sum_{t} \log(n(t)!) + \sum_{t}  \sum_{i=1}^m \left[ x_{i, t} \log p_i(t) - \log(x_{i, t}!) \right] + \sum_{t} \lambda_t (1 - \sum_{i=1}^{m(t)} p_i(t)) \\
    & \max_{\theta} \sum_{t} \log(n(t)!) + \sum_{t} \sum_{i=1}^m \left[ x_{i, t} (\log c_i + p \log t) - \log(x_{i, t}!) \right] + \sum_{t} \lambda_t (1 - \sum_{i=1}^{m(t)} c_i t^p)
\end{align*}

... too many constraints ...

Critical point:

\begin{align*}
\sum_{t} \frac{x_{i, t}}{c_i} - \sum_{t} \lambda_t t^p
    &= 0 \\
\sum_{t} \sum_{i=1}^m x_{i, t} \log t - \sum_{t} \lambda_t \sum_{i=1}^m p c_i t^{p-1}
    &= 0 \\
\end{align*}

Try 4 lognormal multiplicative error:

$$X_i(t) \sim \text{Lognormal}(\log(c_i t^{p}), )$$

What works (?):

$$\E \left[ X_i(t) \right] = c_i t^{p}$$

$$\E \left[ \sum_{i=1}^m X_i(t) \right] = t^{p} \sum_{i=1}^m c_i$$

$$\log \sum_{i=1}^m X_i(t) = p t + \log \sum_{i=1}^m c_i + \eps$$

$$\E \left[ \calX(t) \right] = t^{p} \sum_{i=1}^m c_i$$

$$\E \left[ X_i(T) \; | \; x_{i, :t} \right] = c_i = \frac{x_{i, t}}{t^p}$$

What to consider:

Per-group growth
\begin{enumerate}
    \item Different portions
    % \item (Assumption) if $a > b$ at some $t_0$, $a > b$ at all $t$
\end{enumerate}

Growing groups
\begin{enumerate}
    \item $\frac{1}{m(t)} \sum_{i=1}^{m(t)} X_i(t) = \frac{n(t)}{m(t)}$
\end{enumerate}

==> sections/5_inference.tex <==
% \newpage

\section{Aggregate Inference}
\label{sec:inference}

% \subsection{High-level Approach}

% \begin{enumerate}
% \item Definition: (input dfs) and (output df); time series prediction over structured data
% \item Cases we need to address
% \item Our technique
% \item Accuracy guarantee
% \end{enumerate}

Aggregate inference takes intrinsic states and produces extrinsic states. To do so, it needs to address two complications.
1) The number of samples that contributes to an aggregate may grows non-trivially as \system processes more partitions, rather than trivially growing linearly as $ct$ for some constant $c$. For example, filtering and correlation along partitions could deviate the growth. Additionally, the set of groups may expand over time, splitting away samples from equally sized future partitions. 2) \system needs to support many types of aggregations. Aggregate inference should adapt the estimator accordingly to the operation.

To tackle these challenges, \cref{sec:inference-decompose} decomposes aggregate inference into two parts: cardinality estimator (\cref{sec:inference-cardinality}) and aggregate estimators (\cref{sec:inference-aggregate}).

\subsection{Problem Decomposition}
\label{sec:inference-decompose}

\system formulates aggregate inference as an unbiased estimation problem. Using intrinsic states up until current progress $0 \leq t \leq 1$, aggregate inference aims to find per-cell unbiased estimators at final progress $T = 1$. Suppose the data frame has $m(t)$ groups, $X_i(t)$ denotes the $i$-th group cardinality (i.e. the count of samples belonging to the $i$-th group) at progress $t$. Although many aggregate attributes may be present, aggregate inference focuses on each attribute at a time, referring to the aggregate values of the $i$-th group as $Y_i(t)$. Because unobserved partitions are unknown to \system, $m(t)$, $X_i$, and $Y_i$ are stochastic processes over ``time'' $t$. We write the observed group cardinalities and aggregate values until progress $t$ in lowercases: $x_{i, :t}$ and $y_{i, :t}$ respectively. The desired unbiased estimator $\yh_{i, :t}$ is the one such that:
\begin{equation}
    \yh_{i, :t} = \E \left[ Y_i(T) \; | \; x_{i,:t}, y_{i,:t} \right]
\end{equation}

Many known aggregate estimators rely on the current count $x_{i, t}$ and the final count $x_{i, T}$; however, the latter is not known at the current time. Instead, \system computes an unbiased estimator of final group cardinality $\xh_{i, :t}$ from group cardinalities so far $x_{i, :t}$ described in \cref{sec:inference-cardinality}.
\begin{equation}
    \xh_{i, :t} = \E \left[ X_i(T) \; | \; x_{i, :t} \right]
\end{equation}

Using this estimator as well as the current cardinality and aggregate value, \system then estimates the final aggregate value at $T$ by aggregate-aware estimators $f$ in \cref{sec:inference-aggregate}.
\begin{equation}
    \yh_{i, :t} = \E \left[ Y_i(T) \; | \; x_{i,:t}, y_{i,:t} \right] = f(y_{i,:t},  x_{i, :t}, \xh_{i, :t})
\end{equation}

Therefore, \system first estimates $\xh_{i, :t}$ for all $i = 1, \dots, m(t)$, and then estimates $\yh_{i, :t}$. In a case of many aggregate attributes, \system reuses $\xh_{i, :t}$ to estimate each aggregate separately by applying corresponding aggregate estimator. Finally, it collects all aggregate estimations into the output data frame filled with extrinsic states.

\subsection{Cardinality Estimator}
\label{sec:inference-cardinality}

\system models group cardinalities after monomials with a shared power, $\E[X_i(t)] \propto t^w$. The underlying reasoning is as followed. \system assumes that number of samples and number of groups follow two hidden monomials, $\E[n(t)] \propto t^{u}$ and $\E[m(t)] \propto t^{v}$ respectively. Subsequently, average group cardinality is $\frac{1}{m(t)} \sum_{i=1}^{m(t)} X_i(t) = \frac{1}{m(t)} n(t)$ whose expectation is proportional to $t^{u - v}$ and so we can set $w = u - v$. This modeling captures many scenarios in Deep OLA. For example, if the input data frame is a table reader, then \system would expect the sample to grow linearly ($u = 1$). If the input is behind a cross join of two tables, then \system would expect a quadratic growth ($u = 2$). Filtering would then affect the coefficient corresponding to its selectivity. On the other hand, if the group key is the same as the clustering key, \system would see the number of groups grows linearly ($v = 1$) as it consumes more partitions. A low-cardinality group key would result in a constant ($v = 0$) while a higher-cardinality one would generate something in between ($0 < v \leq 1$). 

Furthermore, the model simplifies its estimation logic. In fact, \system does not need to estimate $\E[n(t)]$ nor $\E[m(t)]$, but only $\E[X_i(t)]$. \system estimates all final group cardinalities in two steps. First, it fits $w$ to the dataset consisting of average group cardinalities $\overline{x}_t = \frac{1}{m_t} \sum_{i=1}^{m_t} x_{i, t}$ for all observed $t$. In particular, it fits the power $w$ as well as the coefficient $b$ in a logarithmic-transformed linear regression: $\E[\log \overline{x}_t] = \log b + w \log t$. \system implements a streaming linear regression which has $O(1)$ time and space complexity per observation. Finally, \system then fits the each group's coefficient in $\E[X_i(t) | x_{i, :t}] = x_{i, t} = c_i t^w$ and predicts the final group cardinality by evaluating at $T = 1$:
\begin{equation}
    \xh_{i, :t} = \E[X_i(T) | x_{i, :t}] = \frac{x_{i, t}}{t^w} T^w = \frac{x_{i, t}}{t^w}
\end{equation}

\subsection{Aggregate Estimators}
\label{sec:inference-aggregate}

\system selects the aggregate estimator $f$ from the following the set of estimators depending on the aggregation type. This set can be expanded together with existing estimators.

\paragraph{Count} Use the estimated cardinality: $f_{\text{count}}(y_{i,:t}, x_{i,:t}, \xh_{i, :t}) = \xh_{i, :t}$.

\paragraph{Summation} Scale the summation: $f_{\text{sum}}(y_{i,:t}, x_{i,:t}, \xh_{i, :t}) = \frac{y_{i,t}}{x_{i,t}} \xh_{i, :t}$.

\paragraph{Weighted averages} Weighted averages (e.g., average, variance, standard deviation) are special cases of summation. Because of our choice of estimators, average estimators reduce to the identity function. Let $y'_{i,:t}$ be the weighted summation, $y''_{i,:t}$ be the summation of weights and $y_{i,t} = y'_{i,t} / y''_{i,t}$ be the weighted average:
\begin{equation}
    f_{\text{avg}}((y'_{i,:t}, y''_{i,:t}), x_{i,:t}, \xh_{i, :t}) = \left( \frac{y'_{i,t}}{x_{i,t}} \xh_{i, :t} \right) / \left( \frac{y''_{i,t}}{x_{i,t}} \xh_{i, :t} \right) = y_{i,t}
\end{equation}

\paragraph{Count distinct} \system adopts the finite-population method-of-moment estimator from~\cite{Haas1995Distinct} (in section 4.1, denoted as $\hat{D}_{MM1}$). For brevity in this subsection, let us focus on $i$-th group and shorten the notations of current group cardinality $x = x_{i,t}$, final estimated group cardinality $X = \xh_{i, :t}$, and current group count distinct $y = y_{i, t}$. \system computes $f_{cd}(y_{i,:t}, x_{i,:t}, \xh_{i, :t}) = Y$ where $Y$ satisfies \cref{eq:mm1-main}.
\begin{equation} \label{eq:mm1-main}
    y_{i, t} = Y ( 1 - h(\xh_{i, :t} / Y) )
\end{equation}

$h(z)$ is defined below. To solve the equation, \system runs Newton-Raphson iterations until convergence with a tolerance and at most a finite number of steps. Each iteration involves evaluating numerical approximation of gamma and digamma functions.
\begin{equation}
    h(z) = \frac{\Gamma(\xh_{i, :t} - z + 1) \Gamma(\xh_{i, :t} - x_{i,t} + 1)}{\Gamma(\xh_{i, :t} - x_{i,t} - z + 1) \Gamma(\xh_{i, :t} + 1)}
\end{equation}

\paragraph{Order statistics} Order statistics include minimum, maximum, median, quantiles, and k-th smallest/largest values. Currently, \system simply outputs the latest value: $f_{\text{order}}(y_{i,:t}, x_{i,:t}, \xh_{i, :t}) = y_{i,t}$ which provides a fairly accurate estimate for large $\xh_{i,:t}$ at no computation cost.


\subsection{Correctness}
\label{sec:inference-analysis}

Given observations $(y_{i,:t}, x_{i,:t})$ up until current progress $t$, \cref{lemma:unbiased-count} and \cref{lemma:unbiased-agg} together show that \system's aggregate inference is unbiased under some conditions.

\begin{lemma} \label{lemma:unbiased-count}
    $\xh_{i, :t} = \E[X_i(T) | x_{i, :t}] = \frac{x_{i,t}}{t^w}$ is unbiased, if A) $w$ is unbiased and B) all operations produce a monomial or transform a monomially growing input(s) into a monomially growing output with respect to progress $t$.
\end{lemma}
\begin{proof}
    To justify A), $w$ is unbiased if a sufficient condition holds: $\overline{X}_t = \frac{1}{m} \sum_{i=1}^{m(t)} X_i(t) = c_i t^w e^\eps$ where $e^\eps$ is a multiplicative error with $\E[\eps] = 0$ and independence to observations. Notice that $\log \overline{X}_t = \log c_i + w \log t + \eps$. By an unbiasedness of ordinary least square estimator, the estimated $w$ coincides with the expectation of $w$.

    To justify B), we show that all operations in \cref{sec:model} can satisfy the property possibly with some additional conditions depending on the operation. First, a data source produces monomial rows by implementation since it computes progress $t$ from the number of rows read divided by the final number of rows. Mapping trivially preserves the cardinality. Joins and filters preserve monomial relationship if each tuple has uniform selectivity and the selectivity is independent from the progress. Lastly, aggregation preserves monomial relationship if the groupby key is either uniformly distributed across progress or is a clustered key.
    
    If B) holds, $\E[X_i(t)] = c_i t^w$ for all \mdf including the input to the aggregation. Because \system has already observed $x_{i, t}$ at $t$, $\E[X_i(t) | x_{i,:t}] = \E[X_i(t) | x_{i,t}] = x_{i, t}$, implying $c_i = x_{i,t} / t^w$ and leading to \system's group cardinality estimator when evaluated at $t = T = 1$.
\end{proof}

\begin{lemma} \label{lemma:unbiased-agg}
    Given the unbiased group cardinality estimate $\xh_{i, :t} = \E[X_i(T) | x_{i, :t}]$, \system's aggregate estimators produce unbiased estimates, possibly with additional conditions depending on aggregation type: $\E \left[ Y_i(T) \; | \; x_{i,:t}, y_{i,:t} \right] = f(y_{i,:t},  x_{i, :t}, \xh_{i, :t})$.
\end{lemma}
\begin{proof}
    This is true for $f_{count}$ because $\xh_{i, :t}$ is given.
    
    Assuming the terms $\{U_{i,j}\}_{j=1}^{X_i(t)}$ in summation are stationary with a constant $\E[U_{i,j}] = \E[U_i]$, $f_{sum}$ is unbiased. Let $Y_i(t) = \sum_{j=1}^{X_i(t)} U_{i,j}$, we can use stationarity to factor $\E[Y_i(T) \; | \; x_{i,:t}, y_{i,:t}] = \E[X_i(T) \; | \; x_{i,:t}] E[U_i \; | \; x_{i,:t}, y_{i,:t}]$. By expanding the conditional expectation, $E[U_i \; | \; x_{i,:t}, y_{i,:t}] = \frac{y_{i,t}}{x_{i,t}}$ which equates the final result to $f_{sum}$.
    
    Assuming that elements and weights are independent, weighted average estimate $f_{avg}$ is unbiased by expectation linearity.
    
    Assuming equal-frequency assumption (i.e. samples are uniformly distributed into $Y$ distinct values), $f_{cd}$ is an unbiased estimator as described in~\cite{Haas1995Distinct}. Additionally, the same work also derives an estimator for skewed frequency, left for future improvements and experiments.

    The $q$-th sample quantile is asymptotically normal around the $q$-th population quantile with variance $q(1-q) / (X_i(t) p_q^2)$ where $p_q$ is the density of the quantile value studied in section 21.2 of~\cite{Vaart1998AsympStats}. Assuming sufficiently large sample size $x_{i,t} = \omega(1/p_q^2)$, which is typical in OLA due to its data size, the sample quantile is unbiased with small variance.
\end{proof}

% \supawit{TODO: extended correctness by subgaussian algebra, assert that we don't actually compute confidence bound}

% \supawit{TODO: secondary consideration: performance, all operations are $O(1)$ per cell, alternatives would need to avoid looking at all input data frame}

\subsection{Alternatives}
\label{sec:inference-alternative}

This section lists some of alternative design choices we have considered but do not fit well with the broader picture of \system.

\paragraph{Probabilistic cardinality estimator} One could model the distribution $X_i(T) | x_{i,:t}$ (instead of the expectation $\E[X_i(T) | x_{i,:t}]$ in \system) to better estimate the aggregate. However, the evaluation would require computing the marginal expectation which may be expensive for many aggregate estimators. Even so, which distribution to use is an open question to be investigated further.

% \paragraph{Dynamic group distribution} \supawit{TODO: when group comes and go, non-monotonic}

% \paragraph{Grammatical cardinality estimator} One could select an estimator at data source nodes (such as data reader) and propagate estimators through operations using a grammar. However, many rules require careful consideration especially those around join and aggregation operations. It would also add complexity to the implementation.

\paragraph{Other cardinality function families} Different families of polynomials are attractive alternatives; however, one need to know the set of orders a priori to efficiently fit the polynomial coefficients. Mixing exponential and logarithm could improve the accuracy in some cases but would also be more difficult to estimate. On the other hand, affine functions are simple with many well-known estimation algorithms, but they are only restricted to a specific growth pattern. Ultimately, monomial is the simplest and cheap to fit (in logarithmic scale) yet provides a wide range of growth curve.

% \paragraph{Multi-attribute estimator} \supawit{TODO: correlate different columns, e.g. VAR}

\paragraph{Unbiased order statistics under finite population} Given probability density function (PDF) and cumulative density functions (CDF), there exists a density function of the $k$-th order statistic~\cite{david2004order}. Given order statistic density function, we could evaluate the expectation at $\xh_{i, :t}$ numerically to acquire the unbiased estimate. Similar analysis is possible for discrete variables as well. However, this method has a prohibitive computation cost in general to reconstruct PDF and CDF, let alone evaluating the expectation. For example, if the reconstruction uses kernel density estimation (KDE)~\cite{rosenblatt1956remarksKDE,parzen1962estimationKDE} and empirical distribution function (eCDF), it would require $O(n(t))$ time and space to compute the density and hold all samples. Such a cost does not scale well and may straggle OLA progress if the accuracy gain is minimal.





% This is a figure for the next section
% \input{figures/fig_architecture}
\input{figures/fig_implementation}








==> sections/a1_edf_closure.tex <==
\section{Closure of Evolving Data Frame}
\label{sec:appendix-closure}

\supawit{For all edfs, all operators map them into another edf.}




==> sections/interface.tex <==
\section{Programming Interface}
\label{sec:interface}



